The Impact of Recommendation Systems on Opinion Dynamics: Microscopic versus Macroscopic Effects

Recommendation systems are widely used in web services, such as social networks and e-commerce platforms, to serve personalized content to the users and, thus, enhance their experience. While personalization assists users in navigating through the available options, there have been growing concerns regarding its repercussions on the users and their opinions. Examples of negative impacts include the emergence of filter bubbles and the amplification of users' confirmation bias, which can cause opinion polarization and radicalization. In this paper, we study the impact of recommendation systems on users, both from a microscopic (i.e., at the level of individual users) and a macroscopic (i.e., at the level of a homogenous population) perspective. Specifically, we build on recent work on the interactions between opinion dynamics and recommendation systems to propose a model for this closed loop, which we then study both analytically and numerically. Among others, our analysis reveals that shifts in the opinions of individual users do not always align with shifts in the opinion distribution of the population. In particular, even in settings where the opinion distribution appears unaltered (e.g., measured via surveys across the population), the opinion of individual users might be significantly distorted by the recommendation system.

==> old/additional_case_study.tex <==

\subsection{Does polarization penetrate through the population?}

In our second analysis, we investigate if and to what extent a polarized recommendation distribution leads to a polarized opinion distribution. For this case study, we consider a population with $\beta=0.8$ and initial opinion uniformly distributed between $-2$ and $2$. Recommender systems have, as above, exploration parameter $T\in\{1,\ldots,21\}$ and the recommendations distributed according to a mixture of Gaussians with standard deviation $0.1$ and mean $\pm \alpha/2$, with $\alpha\in\{0,0.1,\ldots,2\}$ (see~\cref{.}). For each setting, we perform 20 exploration cycles. 
This way, $\weightopinion^{T-1}$, the key quantity revealed by our first case study, varies between $0.01$ and $1.0$, and the distance between the two modes of the polarized recommendation distribution is $\alpha$.

\begin{figure}[bt]
    \centering 
    \begin{tikzpicture}
    \begin{axis}[name=one,
                 colorbar, colorbar style={width=0.2cm,xshift=-0.3cm},
                 width=4.4cm, height=4.4cm,
                 view={0}{90},
                 point meta min=0, %point meta max=0.7,
                 xlabel={$\weightopinion^{T-1}$},
                 %xmin=1, xmax=21,
                 %xtick={1,6,...,19},
                 ylabel={$\alpha$}, ylabel style={yshift=-0.15cm},
                 ymin=0, ymax=2,
                 ytick={0,0.4,...,2},
                 shader=interp,
                 colormap/viridis,
                 %mesh/ordering=x varies,
                 ]
    \addplot3[surf,mesh/cols=20] table [x expr=\thisrowno{0}, y expr=\thisrowno{1}, z expr=\thisrowno{2}, col sep=comma] {figures/dpol.csv}; 
    \end{axis}
    \end{tikzpicture}
    \caption{\ldots For this simulation, we use the same setting as in~\cref{subsec:model:simulation}.}
    \label{fig:noexploration}
\end{figure}

==> old/mycommands.tex <==
% Basic
\newcommand{\naturals}                       {\mathbb{N}}
\newcommand{\reals}                          {\mathbb{R}}
\newcommand{\realsBar}                       {\bar{\mathbb{R}}}
\newcommand{\nonnegativeReals}               {\mathbb{R}_{\geq 0}}
\newcommand{\nonnegativeRealsBar}            {\bar{\mathbb{R}}_{\geq 0}}
\newcommand{\positiveReals}                  {\mathbb{R}_{> 0}}
\newcommand{\cardinality}[1]                 {|#1|}
\newcommand{\identity}[1]                    {\mathrm{Id}_{#1}}
\DeclareMathOperator{\Id}                    {Id}
\DeclareMathOperator{\id}                    {id}
\DeclareMathOperator{\proj}                  {proj}
\newcommand{\projection}[2]                  {\proj_{#1}\left[#2\right]}
\newcommand{\domain}[1]                      {D(#1)}
\newcommand{\effectiveDomain}[1]             {D(#1)}
\newcommand{\onotation}[1]                   {o(#1)}
\newcommand{\st}                             {\,|\,}
\newcommand{\conv}                           {\ast}
\newcommand{\isomorphic}                     {\simeq}
\DeclareMathOperator{\dist}                  {dist}

% Topology
\newcommand{\boundary}[1]                    {\partial #1}
\newcommand{\closure}[1]                     {\overline{#1}}
\newcommand{\sphere}[1]                      {\mathbb{S}^{#1}}

% Linear algebra
\newcommand{\innerProduct}[2]                {\left\langle #1,#2\right\rangle}
\newcommand{\norm}[1]                        {\left\Vert #1\right\Vert}
\newcommand{\ones}[1]                        {\mathbbm{1}_{#1}}
\newcommand{\zeros}[1]                       {\mathds{O}_{#1}}
\newcommand{\eye}[1]                         {I_{#1}}
\DeclareMathOperator{\trace}                 {trace}
\DeclareMathOperator{\rank}                  {rank}
\DeclareMathOperator{\spec}                  {spec}
\let\span\relax
\DeclareMathOperator{\span}                  {span}
\newcommand{\transpose}[1]                   {{#1}^\top}
\newcommand{\minEigenvalue}[1]               {\lambda_\mathrm{min}(#1)}
\newcommand{\maxEigenvalue}[1]               {\lambda_\mathrm{max}(#1)}
\newcommand{\spectralRadius}[1]              {\rho(#1)}

% Probability
\newcommand{\expectedValue}[2]               {\mathbb{E}^{#1}\left[#2\right]}
\DeclareMathOperator{\var}{Var}
\newcommand{\variance}[2]                    {\var^{#1}\left[#2\right]}
\newcommand{\diracMeasure}[1]                {\delta_{#1}}

% Spaces
\newcommand{\spaceProbabilityMeasures}[1]    {\mathcal{P}(#1)}
\newcommand{\Pp}[2]                          {\mathcal{P}_{#1}(#2)}
\newcommand{\Ppabs}[2]                       {\mathcal{P}_{#1,\mathrm{abs}}(#2)}
\newcommand{\spaceMeasures}[1]               {M(#1)}

% Wasserstein 
\newcommand{\wassersteinDistance}[3]         {W_{#1}(#2,#3)}
\newcommand{\wassersteinBall}[3]             {B_{#2}(#3)}
\newcommand{\closedWassersteinBall}[3]       {\bar B_{#2}(#3)}
\newcommand{\setPlans}[2]                    {\Gamma(#1,#2)}
\newcommand{\setOptimalPlans}[2]             {\Gamma_o(#1,#2)}
\newcommand{\optMap}[2]                      {T_{#1}^{#2}}

% Measure theory 
\newcommand{\pushforward}[1]                 {#1_{\#}}
\newcommand{\lebesgueMeasure}[1]             {\mathcal{L}^{#1}}
\renewcommand{\ae}                           {\text{ a.e.}}

% Differential calculus
\renewcommand{\d}[0]                         {\mathrm{d}}
\newcommand{\dx}                             {\d x}
\newcommand{\diff}[2]                        {\frac{\d #1}{\d #2}}
\newcommand{\partialdiff}[2]                 {\frac{\partial #1}{\partial #2}}
\newcommand{\gradient}[1]                    {\nabla_{#1}}
\newcommand{\hessian}[1]                     {\nabla^2_{#1}}
\newcommand{\subdifferential}[1]             {\partial^{-}#1}
\newcommand{\superdifferential}[1]           {\partial^{+}#1}
\DeclareMathOperator{\tangent}               {Tan}
\newcommand{\tangentBundle}[2]               {\tangent_{#1}#2}
\newcommand{\tangentSpace}[2]                {\tangent_{#1}#2}
\newcommand{\lyapunovFunction}[1]            {\Psi_{#1}}
\newcommand{\lieDerivative}[2]               {\mathcal{L}_{#1}[#2]}
\let\div\relax
\DeclareMathOperator{\div}                   {div}

% Convergence
\newcommand{\weakconvergence}[0]             {\rightharpoonup}
\newcommand{\narrowconvergence}[0]           {\rightharpoonup}
\newcommand{\strongconvergence}[0]           {\to}
\newcommand{\weakstarconvergence}[0]         {\overset{\ast}{\rightharpoonup}}

% Function spaces
\newcommand{\spaceSquareIntegrable}[2]       {L^2(#1,#2)}
\newcommand{\Lp}[2]                          {L^{#1}\ifstrempty{#2}{}{(#2)}}
\newcommand{\Lploc}[2]                        {L_\mathrm{loc}^{#1}\ifstrempty{#2}{}{(#2)}}
\newcommand{\LpNorm}[3]                      {\left\Vert #1\right\Vert_{L^{#2}(#3)}}
\newcommand{\absolutelyContinuous}[3]        {\mathrm{AC}^{#1}(#2,#3)}
\newcommand{\localAbsolutelyContinuous}[3]   {\mathrm{AC}_\mathrm{loc}^{#1}(#2,#3)}
\newcommand{\Cc}[1]                          {C_c(#1)}
\newcommand{\Ccinf}[1]                       {C_c^\infty(#1)}
\newcommand{\Cb}[1]                          {C_b\ifstrempty{#1}{}{(#1)}}
\newcommand{\C}[2]                           {C^{#1}\ifstrempty{#2}{}{(#2)}}
\newcommand{\Czero}[1]                       {C^{0}\ifstrempty{#1}{}{(#1)}}
\newcommand{\Cone}[1]                        {C^{1}\ifstrempty{#1}{}{(#1)}}
\newcommand{\Ctwo}[1]                        {C^{2}\ifstrempty{#1}{}{(#1)}}
\newcommand{\Cinf}[1]                        {C^{\infty}\ifstrempty{#1}{}{(#1)}}
\newcommand{\Wr}[2]                          {W^{1,#1}\ifstrempty{#2}{}{(#2)}}
\newcommand{\Wrloc}[2]                       {W^{1,#1}_\mathrm{loc}\ifstrempty{#2}{}{(#2)}}
\newcommand{\Hone}[1]                        {H^{1}\ifstrempty{#1}{}{(#1)}}
\newcommand{\Wrg}[3]                         {W^{1,r}_{#2}\ifstrempty{#3}{}{(#3)}}

% Groups
\DeclareMathOperator{\SOGroup}               {SO}
\newcommand{\SOn}[1]                         {\SOGroup(#1)}

% Category theory
\newcommand{\transportCategory}              {\mathsf{Transp}}
\newcommand{\posetCategory}                  {\mathsf{Pos}}
\newcommand{\setCategory}                    {\mathsf{Set}}
\DeclareMathOperator{\lu}{lu}
\DeclareMathOperator{\ru}{ru}
\DeclareMathOperator{\as}{as}
\newcommand{\objects}[1]                     {\mathsf{Ob}_{#1}}
\DeclareMathOperator{\Hom}                   {Hom}
\newcommand{\comp}[2]                        {#1 \fatsemi #2}

% Comments
\newcommand{\nlmargin}[2]{\margincomment{#1}{#2}{blue}{NL}}
\newcommand{\fdmargin}[2]{\margincomment{#1}{#2}{red}{FD}}
\newcommand{\sbmargin}[2]{\margincomment{#1}{#2}{cyan}{SB}}
